FunQA: Towards Surprising Video Comprehension

Surprising videos, such as funny clips, creative performances, or visual illusions, attract significant attention. Enjoyment of these videos is not simply a response to visual stimuli; rather, it hinges on the human capacity to understand (and appreciate) commonsense violations depicted in these videos. We introduce FunQA, a challenging video question-answering (QA) dataset specifically designed to evaluate and enhance the depth of video reasoning based on counter-intuitive and fun videos. Unlike most video QA benchmarks which focus on less surprising contexts, e.g., cooking or instructional videos, FunQA covers three previously unexplored types of surprising videos: 1) HumorQA, 2) CreativeQA, and 3) MagicQA. For each subset, we establish rigorous QA tasks designed to assess the model's capability in counter-intuitive timestamp localization, detailed video description, and reasoning around counter-intuitiveness. We also pose higher-level tasks, such as attributing a fitting and vivid title to the video and scoring the video creativity. In total, the FunQA benchmark consists of 312K free-text QA pairs derived from 4.3K video clips, spanning a total of 24 video hours. Moreover, we propose FunMentor, an agent designed for Vision-Language Models (VLMs) that uses multi-turn dialogues to enhance models' understanding of counter-intuitiveness. Extensive experiments with existing VLMs demonstrate the effectiveness of FunMentor and reveal significant performance gaps for the FunQA videos across spatial-temporal reasoning, visual-centered reasoning, and free-text generation.

==> sec/6_conclusion.tex <==
\section{Conclusion}
We introduce FunQA, a challenging VideoQA dataset of counter-intuitive and fun videos designed to explore the depth of video reasoning. We established a benchmark of four rigorous tasks and performed a comprehensive evaluation of frontier baselines, which were revealed to demonstrate a significant performance gap compared to manual annotation. Most baselines struggle especially in tasks requiring higher-level reasoning, such as counter-intuitive timestamp localization. We proposed an agent for VLM: FunMentor. It effectively enhances the model's understanding of humor, demonstrating the powerful potential of agent-based finetuning. FunQA dataset and novel benchmark tasks provide valuable insight and future research direction. We expect FunQA to underpin the next generation of VideoQA research that pushes video reasoning beyond superficial descriptions toward deeper understanding. 

==> table/consensus_evaluation.tex <==
\begin{table}[!t]
\begin{minipage}{0.5\linewidth}
\vspace{-0.05mm}
\caption{\textbf{Consensus Evaluation Experiment.} This table shows the results from a random 10\% sample of QA pairs, cross-validated by annotators to assess agreement with existing annotations. `Low,' `Medium,' and `High' indicate the strength of the consensus.}
\label{T:coneval}
\vspace{-10pt}
\centering
\setlength\tabcolsep{8pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
Consensus & HumorQA & CreativeQA & MagicQA & \# Total \\
% \toprule
\hline
Low & 1 & 1 & 2 & 4 \textbf{(1\%)} \\
Medium & 9 & 6 & 17 & 32 \textbf{(8\%}) \\
High & 199 & 111 & 194 & 504 \textbf{(91\%)}\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{minipage}%
\end{table}




==> table/only_frames.tex <==
\begin{table}[!t]
\vspace{-0.05mm}
\caption{\textbf{Can FunQA be Solved Solely Based on Images?} The left two columns show the average number of questions answerable or not by humans using only 8 static, uniformly selected frames.}
\label{T:onlyframes}
\vspace{-10pt}
\centering
\setlength\tabcolsep{15pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc}
\toprule
Dataset  & \# Can & \# Cannot & Cannot Rate($\%$)  \\
% \toprule
\hline
HumorQA & 7.8 & 32.2 & 80 \\
CreativeQA & 6.1 & 33.9 & 85 \\
MagicQA & 2.6 & 37.4 & 94 \\
\midrule
\textbf{FunQA} & 16.5 & 103.5 & \textbf{86} \\
\bottomrule
\end{tabular}
}
\vspace{-5pt}
\end{table}


% \begin{table}[!t]
% \vspace{-0.05mm}
% \caption{\textbf{Can FunQA be Solved Solely Based on Images?} }
% \label{T:onlyframes}
% \vspace{-10pt}
% \centering
% \setlength\tabcolsep{15pt}
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{l|cc}
% \toprule
% Dataset  & # Can & # Cannot & ($\%$)  \\
% % \toprule
% \hline
% HumorQA & 7.8 & 32.2 & 80 \\
% CreativeQA & 6.1 & 33.9 & 85 \\
% MagicQA & 2.6 & 37.4 & 94 \\
% \textbf{FunQA} & 16.5 & 103.5 & \textbf{86} \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

==> table/statics.tex <==
% static table----------------------------
\begin{table}[!t]
\centering
\caption{\textbf{Statistics of the FunQA dataset.}
\label{T:statics}}
\resizebox{0.8\linewidth}{!}{

\begin{tabular}{lccccccc}
\hline
\multirow{2}{*}{Datase} & \multicolumn{4}{c}{Videos} & \multirow{2}{*}{Avg len(s)} & \multirow{2}{*}{Total len(h)} & \multirow{2}{*}{\# QA Pairs} \\ \cline{2-5}
           & Train & Val & Test & Total &    &       &       \\ \hline
HumorQA    & 1,244  & 350 & 172  & 1,769  & 7  & 3.72  & 141,250  \\
CreativeQA & 657   & 185 & 85   & 927   & 48 & 12.53 & 78,740  \\
MagicQA    & 1,171  & 334 & 167  & 1,672  & 16 & 7.65  & 91,960  \\ \hline
FunQA      & 3,072  & 869 & 424  & 4,365  & 19 & 23.90 & 311,950 \\ \hline \\
\end{tabular}
}
\end{table}
%static table ----------------------------------
